Towards Fair and Comprehensive Comparisons for Image-Based 3D Object Detection

In this work, we build a modular-designed codebase, formulate strong training recipes, design an error diagnosis toolbox, and discuss current methods for image-based 3D object detection. In particular, different from other highly mature tasks, e.g., 2D object detection, the community of image-based 3D object detection is still evolving, where methods often adopt different training recipes and tricks resulting in unfair evaluations and comparisons. What is worse, these tricks may overwhelm their proposed designs in performance, even leading to wrong conclusions. To address this issue, we build a module-designed codebase and formulate unified training standards for the community. Furthermore, we also design an error diagnosis toolbox to measure the detailed characterization of detection models. Using these tools, we analyze current methods in-depth under varying settings and provide discussions for some open questions, e.g., discrepancies in conclusions on KITTI-3D and nuScenes datasets, which have led to different dominant methods for these datasets. We hope that this work will facilitate future research in image-based 3D object detection. Our codes will be released at \url{https://github.com/OpenGVLab/3dodi}

==> sections/Benchmark.tex <==
\section{Benchmark}

% Image-based object detection is a complicated perception system and is affected by lots of factors. It is impractical to thoroughly benchmark each of them, and we mainly focus on the following aspects in this work. 


% \noindent
% {\bf Training recipes.}



% \subsection{Datasets and Metrics}

% \noindent
% {\bf KITTI-3D.}
% %We conduct the experiments on the most commonly used KITTI-3D dataset \cite{kitti} and the large-scale nuScenes dataset \cite{nuscenes}. In particular, 
% KITTI-3D \cite{kitti} contains 7,481 and 7,518 frames for training and testing respectively. Following \cite{3dop,mv3d}, we split the training frames into a training set (3,712 frames) and a validation set (3,769 frames), and conduct the experiments in this split. For each frame, the synchronized LiDAR sweep and stereo pair are provided.
% Following \cite{monodis}, we adopt the ${\rm AP}_{40}$ of 3D detection and Bird's Eye View (BEV) detection as metrics. We mainly focus on the Car category on KITTI, and both 0.7 and 0.5
% IoU thresholds are considered.

% \noindent
% {\bf nuScenes.} nuScenes dataset \cite{nuscenes} provides about 40K annotated frames of 10 categories for the panoramic view. In particular, there are 28,130 frames, 6,019 frames, and 6,008 frames for training, validation, and testing respectively (six images per frame). For evaluation, nuScenes uses a  2D center error (in the ground plane) based AP metric. Furthermore, five true positive
% metrics are also considered, including Average Translation Error (ATE), Average Scale Error (ASE), Average Orientation Error (AOE), Average Velocity Error (AVE), and Average Attribute Error (AAE). Finally, the nuScenes detection score (NDS) is computed by weighted averaging the above metrics.

\input{tables/implementation}



\noindent
{\bf Data augmentation.}


\noindent
{\bf Training schedule.}


==> sections/Discussion.tex <==
\section{Discussions}

\subsection{Conflicts in KITTI and nuScenes}

\noindent
{\bf Backbones.}


\noindent
{\bf Data scales.}



\noindent
{\bf Evaluation metrics.}
